The Rumble in the Meson: a leptoquark versus a $Z^\prime$ to fit $b \rightarrow s \mu^+ \mu^-$ anomalies including 2022 LHCb $R_{K^{(\ast)}}$ measurements

We juxtapose global fits of two bottom-up models (an $S_3$ scalar leptoquark model and a ${B_3-L_2}$ $Z^\prime$ model) of \bsll\ anomalies to flavour data in order to quantify statistical preference or lack thereof. The leptoquark model couples directly to left-handed di-muon pairs, whereas the $Z^\prime$ model couples to di-muon pairs with a vector-like coupling. $B_s-\overline{B_s}$ mixing is a focus because it is typically expected to disfavour $Z^\prime$ explanations. In two-parameter fits to 247 flavour observables, including $B_{s/d} \to \mu^+ \mu^-$ branching ratios for which we provide an updated combination and LHCb $R_{K^{(\ast)}}$ measurements from December 2022, we show that each model provides a similar improvement in quality-of-fit of $\sqrt{\Delta \chi^2}=3.6$ with respect to the Standard Model. The main effect of the $B_s-\overline{B_s}$ mixing constraint in the $Z^\prime$ model is to disfavour values of the $s_L-b_L$ mixing angle greater than about $5|V_{cb}|$. This limit is rather loose, meaning that a good fit to data does not require `alignment' in either quark Yukawa matrix. No curtailment of the $s_L-b_L$ mixing angle is evident in the $S_3$ model.

==> letter_to_editor.tex <==
Dear Editor

We thank the referee for their report on our manuscript and their helpful
suggestions. We have amended it based on the points that they raise and
believe that it has improved as a result. We hope that the resulting paper is
now suitable for publication in JHEP.

In particular, in response to their numbered points:
\begin{enumerate}
\item
  This was evidently old text that ``slipped through the net'' in our
  rewriting after the recent LHCb analysis of $R_K$ and $R_{K^\ast}$. We have
  changed the statement to: ``The observables in which the measurements are in
  tension with SM 
  predictions involve di-muon  pairs. The new physics state should therefore
  certainly
  couple to di-muon pairs, but in order to agree with the December 2022 LHCb
  measurements $R_K$ and $R_{K^\ast}$, one may also couple it to di-electron
  pairs with a similar strength, although then the scenario may become
  strongly constrained by LEP constraints~\cite{Greljo:2022jac}.''
\item
  We do not understand why these {\tt axodraw} plots didn't come out in the
  referee's version. However, we have taken screenshots and included them in a
  technically different way, which should hopefully sidestep the problem.
\item
  Indeed, this was a typo in [31]. The issue has been fixed.
\item
  Another typo, now fixed.
\item
  This was due to typos in (2.15) and (2.16) - all fixed.
  \end{enumerate}

